A high resolution VLT/FLAMES study of individual stars in the centre of the Fornax dwarf spheroidal galaxy

For the first time we show the detailed late-stage chemical evolution history of small nearby dwarf spheroidal galaxy in the Local Group. We present the results of a high resolution (R$\sim$20000) FLAMES/GIRAFFE abundance study at ESO/VLT of 81 photometrically selected red giant branch stars in the central 25$'$ of the Fornax dwarf spheroidal galaxy. We present abundances of \alfe\ (Mg, Si, Ca and Ti), iron-peak elements (Fe, Ni and Cr) and heavy elements (Y, Ba, La, Nd and Eu). Our sample was randomly selected, and is clearly dominated by the younger and more metal rich component of Fornax which represents the major fraction of stars in the central region. This means that the majority of our stars are 1$-$4 Gyr old, and thus represent the end phase of chemical evolution in this system. Our sample of stars has unusually low [$\alpha$/Fe], [Ni/Fe] and [Na/Fe] compared to the Milky Way stellar populations at the same [Fe/H]. The particularly important role of stellar winds from low metallicity AGB stars in the creation of s-process elements is clearly seen from the high [Ba/Y]. Furthermore, we present evidence for an s-process contribution to Eu.

==> tb-FLAMES-obslog.tex <==
  2003-09-29 &       0&   14400&    6225 \\  
  2003-09-30 &    3600&       0&   14102 \\  
  2003-10-01 &   10800&       0&    6900 \\  
  2004-01-14 &    3600&       0&       0 \\  
  2004-01-15 &       0&    3600&       0 \\  
  2004-01-19 &       0&    7200&       0 \\  
  2004-01-20 &       0&    3600&       0 \\  
  2004-01-21 &       0&       0&    7200 \\  
  2004-01-22 &       0&       0&    7503 \\  
  2004-01-23 &    3600&       0&    3600 \\  
  2004-01-24 &    3600&       0&       0 \\  
  2004-01-26 &    3600&       0&       0 \\  
\hline 
  Total      &      8h&      8h&  12h39m \\  


==> tb-fnx-stelpar_erro.tex <==
\,[Na\,{\sc i}/H] & -0.18&  0.01&  0.01&  0.18\\
\,[Mg\,{\sc i}/H] & -0.06&  0.00&  0.06&  0.08\\
\,[Si\,{\sc i}/H] &  0.14&  0.12&  0.02&  0.19\\
\,[Ca\,{\sc i}/H] & -0.23&  0.04&  0.07&  0.24\\
\,[Ti\,{\sc i}/H] & -0.33&  0.08&  0.04&  0.34\\
\,[Ti\,{\sc ii}/H]&  0.10&  0.21&  0.04&  0.24\\
\,[Cr\,{\sc i}/H] & -0.32&  0.11&  0.09&  0.35\\
\,[Fe\,{\sc i}/H] & -0.04&  0.12&  0.08&  0.15\\
\,[Fe\,{\sc ii}/H]&  0.32&  0.28&  0.04&  0.43\\
\,[Ni\,{\sc i}/H] & -0.03&  0.14&  0.05&  0.15\\
 \,[Y\,{\sc ii}/H]&  0.06&  0.19&  0.02&  0.20\\
\,[Ba\,{\sc ii}/H]& -0.03&  0.15&  0.26&  0.30\\
\,[La\,{\sc ii}/H]& -0.05&  0.23&  0.04&  0.23\\
\,[Nd\,{\sc ii}/H]&  0.00&  0.20&  0.02&  0.20\\
\,[Eu\,{\sc ii}/H]&  0.03&  0.22&  0.04&  0.22\\



==> tb-fnx-vrad.tex <==
    {BL038}&       {  62.86}&     {   0.74}&     {BL147}&       {  52.39}&     {   0.61}&     {BL221}&       {  54.25}&     {   0.32}\\          
    {BL045}&       {  79.54}&     {   0.23}&     {BL148}&       {  65.48}&     {   0.65}&     {BL227}&       {  52.15}&     {   0.67}\\          
    {BL052}&       {  30.32}&     {   1.25}&     {BL149}&       {  50.70}&     {   0.40}&     {BL228}&       {  55.00}&     {   0.34}\\          
    {BL061}&       {  82.38}&     {   1.12}&     {BL150}&       {  68.70}&     {   1.12}&     {BL229}&       {  63.09}&     {   0.57}\\          
    {BL065}&       {  63.86}&     {   0.78}&     {BL151}&       {  41.41}&     {   0.58}&     {BL231}&       {  63.28}&     {   1.11}\\          
 \st{BL069}&    \st{  68.85}&  \st{   2.63}&     {BL153}&       {  50.68}&     {   0.53}&     {BL233}&       {  58.91}&     {   0.40}\\          
 \st{BL070}&    \st{  60.43}&  \st{   2.85}&     {BL155}&       {  46.18}&     {   0.21}&     {BL239}&       {  47.47}&     {   0.35}\\          
    {BL076}&       {  52.83}&     {   0.78}&     {BL156}&       {  30.63}&     {   0.55}&     {BL242}&       {  39.48}&     {   0.55}\\          
    {BL077}&       {  56.23}&     {   1.49}&     {BL158}&       {  41.26}&     {   0.67}&     {BL247}&       {  40.40}&     {   0.63}\\          
    {BL079}&       {  56.31}&     {   0.56}&     {BL160}&       {  53.50}&     {   0.70}&     {BL249}&       {  63.30}&     {   0.73}\\          
    {BL081}&       {  50.58}&     {   0.22}&     {BL163}&       {  41.29}&     {   0.48}&     {BL250}&       {  42.06}&     {   0.36}\\          
    {BL084}&       {  58.92}&     {   0.80}&     {BL165}&       {  70.01}&     {   0.71}&     {BL251}&       {  55.14}&     {   0.45}\\          
 \bf{BL085}&    \bf{  88.97}&  \bf{   1.17}&     {BL166}&       {  57.36}&     {   0.51}&     {BL253}&       {  67.48}&     {   0.39}\\          
    {BL091}&       {  52.79}&     {   0.44}&     {BL168}&       {  75.50}&     {   0.78}&     {BL254}&       {  73.05}&     {   0.26}\\          
    {BL092}&       {  53.99}&     {   0.37}&     {BL171}&       {  58.27}&     {   1.19}&     {BL257}&       {  56.51}&     {   0.36}\\          
    {BL094}&       {  47.45}&     {   0.43}&     {BL173}&       {  44.93}&     {   1.60}&     {BL258}&       {  49.41}&     {   0.79}\\          
    {BL096}&       {  72.90}&     {   0.37}&     {BL180}&       {  72.51}&     {   0.21}&     {BL260}&       {  61.11}&     {   0.70}\\          
    {BL097}&       {  47.47}&     {   0.18}&  \st{BL181}&    \st{  57.46}&  \st{   1.89}&     {BL261}&       {  71.35}&     {   1.27}\\          
    {BL100}&       {  55.92}&     {   0.46}&  \bf{BL183}&    \bf{  19.09}&  \bf{   0.32}&     {BL262}&       {  47.72}&     {   0.52}\\          
    {BL104}&       {  51.36}&     {   0.31}&     {BL185}&       {  55.32}&     {   0.44}&     {BL266}&       {  52.47}&     {   1.43}\\          
    {BL107}&       {  63.97}&     {   0.42}&     {BL189}&       {  82.78}&     {   0.47}&     {BL267}&       {  59.04}&     {   0.48}\\          
 \bf{BL109}&    \bf{ -15.20}&  \bf{   0.42}&     {BL190}&       {  57.31}&     {   0.24}&     {BL269}&       {  45.33}&     {   0.30}\\          
 \st{BL112}&    \st{  53.90}&  \st{   2.36}&     {BL195}&       {  39.03}&     {   0.46}&  \st{BL273}&    \st{  63.77}&  \st{   6.18}\\          
    {BL113}&       {  59.21}&     {   0.31}&     {BL196}&       {  79.09}&     {   0.25}&  \st{BL274}&    \st{  41.22}&  \st{   1.65}\\          
    {BL115}&       {  70.05}&     {   0.30}&     {BL197}&       {  46.27}&     {   1.02}&     {BL278}&       {  52.43}&     {   0.56}\\          
 \st{BL119}&    \st{  56.25}&  \st{   1.95}&  \st{BL198}&    \st{  45.06}&  \st{  11.29}&     {BL279}&       {  67.66}&     {   0.73}\\          
    {BL122}&       {  65.88}&     {   0.75}&     {BL203}&       {  56.40}&     {   0.92}&     {BL293}&       {  56.83}&     {   0.99}\\          
    {BL123}&       {  73.85}&     {   0.71}&     {BL204}&       {  59.30}&     {   0.81}&     {BL295}&       {  42.56}&     {   0.37}\\          
    {BL125}&       {  58.23}&     {   0.77}&     {BL205}&       {  59.91}&     {   0.27}&     {BL298}&       {  62.09}&     {   1.43}\\          
    {BL127}&       {  46.60}&     {   0.67}&     {BL207}&       {  48.82}&     {   0.42}&     {BL300}&       {  69.67}&     {   0.41}\\          
    {BL132}&       {  40.34}&     {   0.48}&     {BL208}&       {  54.35}&     {   0.53}&     {BL304}&       {  71.21}&     {   0.26}\\          
    {BL135}&       {  45.64}&     {   0.57}&     {BL210}&       {  51.51}&     {   0.32}&     {BL311}&       {  50.86}&     {   0.23}\\          
    {BL138}&       {  56.52}&     {   0.33}&     {BL211}&       {  50.35}&     {   0.20}&     {BL315}&       {  53.15}&     {   0.85}\\          
    {BL140}&       {  46.13}&     {   0.69}&     {BL213}&       {  71.82}&     {   0.45}&     {BL323}&       {  52.72}&     {   1.15}\\          
    {BL141}&       {  76.47}&     {   0.35}&     {BL216}&       {  66.92}&     {   0.26}&  \bf{BL325}&    \bf{  18.70}&  \bf{   0.80}\\          
    {BL146}&       {  50.01}&     {   0.61}&     {BL218}&       {  63.33}&     {   0.46}&            &                &              \\

